BEE: Metric-Adapted Explanations via Baseline Exploration-Exploitation

Two prominent challenges in explainability research involve 1) the nuanced evaluation of explanations and 2) the modeling of missing information through baseline representations. The existing literature introduces diverse evaluation metrics, each scrutinizing the quality of explanations through distinct lenses. Additionally, various baseline representations have been proposed, each modeling the notion of missingness differently. Yet, a consensus on the ultimate evaluation metric and baseline representation remains elusive. This work acknowledges the diversity in explanation metrics and baselines, demonstrating that different metrics exhibit preferences for distinct explanation maps resulting from the utilization of different baseline representations and distributions. To address the diversity in metrics and accommodate the variety of baseline representations in a unified manner, we propose Baseline Exploration-Exploitation (BEE) - a path-integration method that introduces randomness to the integration process by modeling the baseline as a learned random tensor. This tensor follows a learned mixture of baseline distributions optimized through a contextual exploration-exploitation procedure to enhance performance on the specific metric of interest. By resampling the baseline from the learned distribution, BEE generates a comprehensive set of explanation maps, facilitating the selection of the best-performing explanation map in this broad set for the given metric. Extensive evaluations across various model architectures showcase the superior performance of BEE in comparison to state-of-the-art explanation methods on a variety of objective evaluation metrics.

==> latex/0_abstract.tex <==
\begin{abstract}


Two prominent challenges in Explainable AI involve 1) the nuanced evaluation of explanations and 2) the modeling of missing information through baseline representations. The existing literature introduces diverse evaluation metrics, each scrutinizing the quality of explanations through distinct lenses. Additionally, various baseline representations have been proposed, each modeling the notion of missingness differently. Yet, a consensus on the ultimate evaluation metric and baseline representation remains elusive. This work acknowledges the diversity in explanation metrics and baselines, demonstrating that different metrics exhibit preferences for distinct explanation maps resulting from the utilization of different baseline representations. To address the diversity in metrics and accommodate the variety of baseline representations in a unified manner, we propose Baseline Exploration-Exploitation (BEE) - a path-integration method that introduces randomness to the integration process by modeling the baseline as a learned random tensor. This tensor follows a distribution optimized through a contextual exploration-exploitation procedure to enhance performance on the specific metric of interest. By resampling the baseline from the learned distribution, BEE generates a comprehensive set of explanation maps, facilitating the selection of the best-performing explanation map for the given metric.
Extensive evaluations across various model architectures showcase the superior performance of BEE in comparison to state-of-the-art explanation methods, across multiple metrics. Our code is available at: \url{https://github.com/cvisionuser/bee}
\end{abstract}

==> latex/tables/ablation_multiple_layers.tex <==
\begin{table*}[ht!]
  \begin{center}

  \scalebox{0.8}{
    \begin{tabular}{c l l l l l l l l l }
    \toprule
      & {$\mathcal{I}$} & {NEG} & {POS} & {INS} & {DEL} & {ADP} & {PIC} & {SIC} & {AIC} \\
    \midrule

        & \multirow{1}{*}{$\mathcal\{L\}$}  & {59.10} & {13.69} & {51.15} & {11.19} & {11.35} & {48.22} & {81.23} & {78.45} \\
        
        & \multirow{1}{*}{$\mathcal\{L, L-1\}$}  &  {59.93}& {12.28} & {51.59} & {10.88} &  {11.18}& {48.79}  & {81.49} & {79.11} \\

        & \multirow{1}{*}{$\mathcal\{L, L-1, L-2\}$}  &  {60.21}& {11.74} & {51.96} & {10.03} &  {10.90}& {49.27}  & {81.85} & {80.43} \\


        \midrule
  \end{tabular}}
  \end{center}
    \caption{Ablation Study: Comparison between different settings of $\mathcal{I}$ - the set of layer indices on which the integration process for pBEE is applied.
  }
  \label{tab:ablation_multiple_layers}
\end{table*}

==> latex/tables/cnn_explanation.tex <==
\begin{table*}[t]
  \centering
   \scalebox{0.8}{
    \begin{tabular}
    {l  l  lc@{}lc@{}lc@{}lc@{}lc@{}lc@{}lc@{}}
    % {@{}l  c @{} | lc@{}lc@{}lc@{}lc@{}lc@{}lc@{}lc@{}}
    \toprule
      &  & \multicolumn{1}{c}{GC} & \multicolumn{1}{c}{GC++} & \multicolumn{1}{c}{LIFT} & \multicolumn{1}{c}{AC} & \multicolumn{1}{c}{IG}& \multicolumn{1}{c}{GIG}& \multicolumn{1}{c}{BIG} & \multicolumn{1}{c}{FG} & \multicolumn{1}{c}{LC} & \multicolumn{1}{c}{IIA} & \multicolumn{1}{c}{pBEE}& \multicolumn{1}{c}{fBEE}\\
    \midrule
    % \multirow{8}{*}{RN}

    & \multirow{1}{*}{NEG} & \multicolumn{1}{c}{56.41} & \multicolumn{1}{c}{55.20} & \multicolumn{1}{c}{55.39} & \multicolumn{1}{c}{54.98} & \multicolumn{1}{c}{45.66} &\multicolumn{1}{c}{43.97} & \multicolumn{1}{c}{42.25}& \multicolumn{1}{c}{54.81} & \multicolumn{1}{c}{53.52} & \multicolumn{1}{c}{56.29} & \multicolumn{1}{c}{\underline{59.10}}& \multicolumn{1}{c}{\textbf{59.38}}  \\


    & \multirow {1}{*}{POS}  & \multicolumn{1}{c}{17.82} & \multicolumn{1}{c}{18.01} & \multicolumn{1}{c}{17.53} & \multicolumn{1}{c}{19.38} & \multicolumn{1}{c}{17.24} &\multicolumn{1}{c}{17.68} & \multicolumn{1}{c}{17.44} & \multicolumn{1}{c}{18.06} & \multicolumn{1}{c}{17.92} & \multicolumn{1}{c}{16.62} & \multicolumn{1}{c}{\underline{13.69}} & \multicolumn{1}{c}{\textbf{13.47}}\\
    

    & \multirow {1}{*}{INS}   & \multicolumn{1}{c}{48.14} & \multicolumn{1}{c}{47.56} & \multicolumn{1}{c}{45.39} & \multicolumn{1}{c}{47.05} & \multicolumn{1}{c}{39.87}  &\multicolumn{1}{c}{37.92} & \multicolumn{1}{c}{36.04}& \multicolumn{1}{c}{42.68} & \multicolumn{1}{c}{46.11} & \multicolumn{1}{c}{48.01} & \multicolumn{1}{c}{\underline{51.15}}& \multicolumn{1}{c}{\textbf{51.73}} \\


    & \multirow {1}{*}{DEL}   & \multicolumn{1}{c}{13.97} & \multicolumn{1}{c}{14.17} & \multicolumn{1}{c}{15.32} & \multicolumn{1}{c}{14.23} & \multicolumn{1}{c}{13.49} &\multicolumn{1}{c}{14.18} & \multicolumn{1}{c}{13.95}& \multicolumn{1}{c}{14.64} & \multicolumn{1}{c}{14.31} & \multicolumn{1}{c}{13.18} & \multicolumn{1}{c}{\underline{11.19}} & \multicolumn{1}{c}{\textbf{10.42}}\\


     & \multirow {1}{*}{ADP}   & \multicolumn{1}{c}{17.87} & \multicolumn{1}{c}{16.91} & \multicolumn{1}{c}{18.03} & \multicolumn{1}{c}{16.18} & \multicolumn{1}{c}{37.52} &\multicolumn{1}{c}{35.28} & \multicolumn{1}{c}{40.85}& \multicolumn{1}{c}{21.06} & \multicolumn{1}{c}{24.34} & \multicolumn{1}{c}{12.79} & \multicolumn{1}{c}{\underline{11.35}}& \multicolumn{1}{c}{\textbf{11.09}}\\



    & \multirow {1}{*}{PIC} &  \multicolumn{1}{c}{36.69} & \multicolumn{1}{c}{36.53} & \multicolumn{1}{c}{35.95} & \multicolumn{1}{c}{35.52} & \multicolumn{1}{c}{19.94} &\multicolumn{1}{c}{18.72} & \multicolumn{1}{c}{24.53}& \multicolumn{1}{c}{31.59} & \multicolumn{1}{c}{35.43} & \multicolumn{1}{c}{42.96} & \multicolumn{1}{c}{\underline{48.22}}& \multicolumn{1}{c}{\textbf{48.86}}\\



    & \multirow {1}{*}{SIC}   &  \multicolumn{1}{c}{76.91} & \multicolumn{1}{c}{76.44} & \multicolumn{1}{c}{76.73} & \multicolumn{1}{c}{73.36} & \multicolumn{1}{c}{54.67} & \multicolumn{1}{c}{55.04} & \multicolumn{1}{c}{56.98} & \multicolumn{1}{c}{75.35} & \multicolumn{1}{c}{73.93} & \multicolumn{1}{c}{78.52} & \multicolumn{1}{c}{\underline{81.23}} & \multicolumn{1}{c}{\textbf{81.51}}\\




        & \multirow {1}{*}{AIC}   &  \multicolumn{1}{c}{74.36} & \multicolumn{1}{c}{71.97} & \multicolumn{1}{c}{72.76} & \multicolumn{1}{c}{70.35} & \multicolumn{1}{c}{51.92} & \multicolumn{1}{c}{53.38} & \multicolumn{1}{c}{53.36} & \multicolumn{1}{c}{71.49} & \multicolumn{1}{c}{65.77} & \multicolumn{1}{c}{75.49} & \multicolumn{1}{c}{\underline{78.45}}& \multicolumn{1}{c}{\textbf{79.21}}\\

           
        \bottomrule
      \end{tabular}}
\caption{Results on the IN dataset for the RN backbone: For POS, DEL and ADP, lower is better. For NEG, INS, PIC, SIC and AIC, higher is better. See Sec.~\ref{subsec:results} for details. }
  \label{tab:cnn_backbones_metrics_exp}
    \end{table*}

==> latex/tables/runtime_comparison.tex <==
\begin{table}
  \centering
 
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Runtime (ms) \\
    \midrule
    IG & 265 \\
    pBEE & 228 \\
    fBEE & 1502\\
    \bottomrule
  \end{tabular}
   \caption{Runtime comparison between IG, pBEE and fBEE.}
  \label{tab:runtime_comparison}
\end{table}

==> latex/tables/vit_explanation_before.tex <==
% \begin{table}

% \caption{\oren{consider rotate this table so it will save space and look different than IIA}Results on the IN dataset (ViT models): For POS, DEL and ADP, lower is better. For NEG, INS, PIC, SIC and AIC, higher is better. See Sec.~\ref{subsec:results} for details.
%   }
%   \label{tab:vit_backbones_metrics_exp}  
%   \begin{center}

%   \scalebox{1}{
%     \begin{tabular}{@{}lc@{}lc@{}lc@{}lc@{}}
%     \toprule
%       & & \multicolumn{1}{l}{T-Attr} & \multicolumn{1}{l}{GAE} & \multicolumn{1}{l}{IIA} & \multicolumn{1}{l}{pBEE}& \multicolumn{1}{l}{fBEE} \\
%     \midrule
%     \multirow{8}{*}{ViT-B}
    
%         & \multirow {1}{*}{NEG} & \multicolumn{1}{l}{{54.16}} & \multicolumn{1}{l}{{54.61}}& \multicolumn{1}{l}{{56.01}} & \multicolumn{1}{l}{\underline{58.19}} & \multicolumn{1}{l}{\textbf{58.35}}\\
            
        
%         & \multirow {1}{*}{POS} &  \multicolumn{1}{l}{17.03} & \multicolumn{1}{l}{17.32}& \multicolumn{1}{l}{{15.19}} & \multicolumn{1}{l}{\underline{12.51}}& \multicolumn{1}{l}{\textbf{12.17}}\\
            

%         & \multirow {1}{*}{INS} & \multicolumn{1}{l}{48.58} & \multicolumn{1}{l}{48.96}& \multicolumn{1}{l}{{49.31}} & \multicolumn{1}{l}{\underline{51.13}}& \multicolumn{1}{l}{\textbf{51.36}}\\
            
        
%         & \multirow {1}{*}{DEL} & \multicolumn{1}{l}{{14.20}} & \multicolumn{1}{l}{{14.37}} & \multicolumn{1}{l}{{12.89}}& \multicolumn{1}{l}{\underline{10.94}}& \multicolumn{1}{l}{\textbf{10.76}}\\
           
%          & \multirow {1}{*}{ADP} & \multicolumn{1}{l}{{54.02}} & \multicolumn{1}{l}{{37.84}}& \multicolumn{1}{l}{{33.93}} & \multicolumn{1}{l}{\underline{29.05}}& \multicolumn{1}{l}{\textbf{28.43}}\\
            
        
%         & \multirow {1}{*}{PIC} & \multicolumn{1}{l}{13.37} & \multicolumn{1}{l}{23.65} & \multicolumn{1}{l}{{26.18}} & \multicolumn{1}{l}{\underline{31.01}}& \multicolumn{1}{l}{\textbf{32.14}}\\
           

%         & \multirow {1}{*}{SIC} & \multicolumn{1}{l}{68.59} & \multicolumn{1}{l}{68.35} & \multicolumn{1}{l}{{68.92}} & \multicolumn{1}{l}{\underline{71.22}} & \multicolumn{1}{l}{\textbf{71.45}}\\
           

%         & \multirow {1}{*}{AIC} & \multicolumn{1}{l}{61.34} & \multicolumn{1}{l}{57.92}  & \multicolumn{1}{l}{{62.38}}& \multicolumn{1}{l}{\underline{65.32}} & \multicolumn{1}{l}{\textbf{66.81}}\\
             
%         \midrule
        
%     \multirow{8}{*}{ViT-S}
    
%         & \multirow {1}{*}{NEG} & \multicolumn{1}{l}{53.29} & \multicolumn{1}{l}{52.81} & \multicolumn{1}{l}{{55.76}} & \multicolumn{1}{l}{\underline{57.74}} & \multicolumn{1}{l}{\textbf{58.07}}\\
            
        
%         & \multirow {1}{*}{POS} & \multicolumn{1}{l}{14.16} & \multicolumn{1}{l}{14.75} & \multicolumn{1}{l}{{13.06}} & \multicolumn{1}{l}{\underline{11.84}}& \multicolumn{1}{l}{\textbf{11.62}}\\
            
        
%         & \multirow {1}{*}{INS} & \multicolumn{1}{l}{45.72} & \multicolumn{1}{l}{45.21}  & \multicolumn{1}{l}{{46.55}}& \multicolumn{1}{l}{\underline{48.66}}& \multicolumn{1}{l}{\textbf{49.33}} \\
            
         
%          & \multirow {1}{*}{DEL} & \multicolumn{1}{l}{11.28} & \multicolumn{1}{l}{11.92} & \multicolumn{1}{l}{{11.18}} & \multicolumn{1}{l}{\underline{9.56}}& \multicolumn{1}{l}{\textbf{9.42}} \\
           
             
%          & \multirow {1}{*}{ADP} & \multicolumn{1}{l}{51.94} & \multicolumn{1}{l}{36.98} & \multicolumn{1}{l}{{36.74}}& \multicolumn{1}{l}{\underline{34.90}} & \multicolumn{1}{l}{\textbf{34.74}}\\
             
        
%         & \multirow {1}{*}{PIC} &   \multicolumn{1}{l}{13.67} &  \multicolumn{1}{l}{8.68}& \multicolumn{1}{l}{{15.49}} & \multicolumn{1}{l}{\underline{22.48}}& \multicolumn{1}{l}{\textbf{24.63}}\\
           

%         & \multirow {1}{*}{SIC} &  \multicolumn{1}{l}{69.46} & \multicolumn{1}{l}{70.19}  & \multicolumn{1}{l}{{70.54}}& \multicolumn{1}{l}{\underline{72.85}}& \multicolumn{1}{l}{\textbf{73.16}}\\
            

%         & \multirow {1}{*}{AIC} &  \multicolumn{1}{l}{63.86} & \multicolumn{1}{l}{64.49}  & \multicolumn{1}{l}{{65.02}}& \multicolumn{1}{l}{\underline{68.29}}& \multicolumn{1}{l}{\textbf{68.44}}\\
            
%         \bottomrule
%   \end{tabular}}

%   \end{center}
%   \vspace{-2mm}
% \end{table}

\begin{table*}
\caption{Results on the IN dataset (ViT models): For POS, DEL, and ADP, lower is better. For NEG, INS, PIC, SIC, and AIC, higher is better. See Sec.~\ref{subsec:results} for details. \yoni{Use only half of this table and put the rest in the appendix.}}
% \vspace{-8mm}
\label{tab:vit_backbones_metrics_exp}
\begin{center}
\scalebox{0.83}{
\begin{tabular}{@{}l|cccccccc|cccccccc@{}}
\toprule
\multicolumn{8}{c}{ViT-B} & \multicolumn{8}{c}{ViT-S} \\
\cmidrule(lr){0-1}\cmidrule(lr){2-9} \cmidrule(lr){10-17}
 & NEG & POS & INS & DEL & ADP & PIC & SIC & AIC & NEG & POS & INS & DEL & ADP & PIC & SIC & AIC \\
\midrule
T-Attr & 54.16 & 17.03 & 48.58 & 14.20 & 54.02 & 13.37 & 68.59 & 61.34 & 53.29 & 14.16 & 45.72 & 11.28 & 51.94 & 13.67 & 69.46 & 63.86 \\
GAE & 54.61 & 17.32 & 48.96 & 14.37 & 37.84 & 23.65 & 68.35 & 57.92 & 52.81 & 14.75 & 45.21 & 11.92 & 36.98 & 8.68 & 70.19 & 64.49 \\
IIA & 56.01 & 15.19 & 49.31 & 12.89 & 33.93 & 26.18 & 68.92 & 62.38 & 55.76 & 13.06 & 46.55 & 11.18 & 36.74 & 15.49 & 70.54 & 65.02 \\
pBEE & \underline{58.19} & \underline{12.51} & \underline{51.13} & \underline{10.94} & \underline{29.05} & \underline{31.01} & \underline{71.22} & \underline{65.32} & \underline{57.74} & \underline{11.84} & \underline{48.66} & \underline{9.56} & \underline{34.90} & \underline{22.48} & \underline{72.85} & \underline{68.29} \\
fBEE & \textbf{58.35} & \textbf{12.17} & \textbf{51.36} & \textbf{10.76} & \textbf{28.43} & \textbf{32.14} & \textbf{71.45} & \textbf{66.81} & \textbf{58.07} & \textbf{11.62} & \textbf{49.33} & \textbf{9.42} & \textbf{34.74} & \textbf{24.63} & \textbf{73.16} & \textbf{68.44} \\ \bottomrule
\end{tabular}}
\end{center}
% \vspace{-2mm}
\end{table*}

